Human-AI Collaborative Uncertainty Quantification

AI predictive systems are increasingly embedded in decision making pipelines, shaping high stakes choices once made solely by humans. Yet robust decisions under uncertainty still rely on capabilities that current AI lacks: domain knowledge not captured by data, long horizon context, and reasoning grounded in the physical world. This gap has motivated growing efforts to design collaborative frameworks that combine the complementary strengths of humans and AI. This work advances this vision by identifying the fundamental principles of Human AI collaboration within uncertainty quantification, a key component of reliable decision making. We introduce Human AI Collaborative Uncertainty Quantification, a framework that formalizes how an AI model can refine a human expert's proposed prediction set with two goals: avoiding counterfactual harm, ensuring the AI does not degrade correct human judgments, and complementarity, enabling recovery of correct outcomes the human missed. At the population level, we show that the optimal collaborative prediction set follows an intuitive two threshold structure over a single score function, extending a classical result in conformal prediction. Building on this insight, we develop practical offline and online calibration algorithms with provable distribution free finite sample guarantees. The online method adapts to distribution shifts, including human behavior evolving through interaction with AI, a phenomenon we call Human to AI Adaptation. Experiments across image classification, regression, and text based medical decision making show that collaborative prediction sets consistently outperform either agent alone, achieving higher coverage and smaller set sizes across various conditions.

==> garbage.tex <==

\iffalse
\newpage
In the offline setting, we assume access to a calibration dataset $\mathcal{D}_{\text{cal}} = \{(X_i, Y_i, H(X_i))\}_{i=1}^n$ that is exchangeable with the test data. 

The thresholds are chosen by computing the empirical quantiles of the scores from the calibration set, conditioned on whether the true label was in the human's set. Let $s_i = 1-p(Y_i|X_i)$ be the score for calibration point $i$. We set:
\begin{align*}
    \hat{b} &= \text{Quantile}_{1-\varepsilon}\Big( \{s_i \mid Y_i \in H(X_i)\} \cup \{\infty\} \Big) \\
    \hat{a} &= \text{Quantile}_{\delta}\Big( \{s_i \mid Y_i \notin H(X_i)\} \cup \{\infty\} \Big)
\end{align*}
The final prediction set for a new test point $X_{\text{test}}$ is then given by $C(X_{\text{test}}) = \{y \mid s(y|X_{\text{test}}) \le \hat{a} \cdot \mathbf{1}\{y \notin H(X_{\text{test}})\} + \hat{b} \cdot \mathbf{1}\{y \in H(X_{\text{test}})\}\}$. This choice of thresholds leads to the following coverage guarantees.

\begin{proposition}[Finite-Sample Offline Guarantees]
Let $(X_{n+1}, Y_{n+1}, H(X_{n+1}))$ be a new test point, exchangeable with the calibration data. Let $n_1$ be the number of calibration points where $Y_i \in H(X_i)$ and $n_2$ be the number where $Y_i \notin H(X_i)$. The thresholds $\hat{a}$ and $\hat{b}$ satisfy:
\begin{align*}
    1-\varepsilon \le \mathbb{P}(Y_{n+1} \in C(X_{n+1}) \mid Y_{n+1} \in H(X_{n+1})) &< 1-\varepsilon + \frac{1}{n_1+1} \\
    \delta \le \mathbb{P}(Y_{n+1} \in C(X_{n+1}) \mid Y_{n+1} \notin H(X_{n+1})) &< \delta + \frac{1}{n_2+1}
\end{align*}
\end{proposition}
\section{Finite sample Online algorithm}\label{online}
In practice, the human may change their behavior over time, adapting to the AI model, and breaking changeability assumption with the calibration data. To handle this, we design an online algorithm that adapts the thresholds $(a_t, b_t)$ round by round so that the long-run error rates converge to their targets.  

At each time step $t$, let $s(y|x) = 1 - p(y|x)$ be the conformity score. We track two kinds of errors:  
\[
\text{err}_{\text{CH},t} := \mathbf{1}\{Y_t \notin C_t(a_t,b_t),\ Y_t \in H(X_t)\}, \quad
\text{err}_{\text{A},t} := \mathbf{1}\{Y_t \notin C_t(a_t,b_t),\ Y_t \notin H(X_t)\}.
\]
The first is a \emph{counterfactual harm} error (we excluded the true label even though the human had it), and the second is an \emph{advantage} error (we excluded the true label when the human missed it).  

The algorithm updates one threshold at a time, depending on whether the human included the true label. If $Y_t \in H(X_t)$, we update $b_t$ to keep the counterfactual harm rate close to $\varepsilon$:  
\[
b_{t+1} = b_t + \eta(\mathbf{1}\{s(Y_t|X_t) > b_t\} - \varepsilon), \qquad a_{t+1} = a_t.
\]
If $Y_t \notin H(X_t)$, we update $a_t$ to keep the advantage rate close to $\delta$:  
\[
a_{t+1} = a_t + \eta(\mathbf{1}\{s(Y_t|X_t) > a_t\} - (1-\delta)), \qquad b_{t+1} = b_t.
\]
Here $\eta>0$ is a learning rate. Intuitively, if errors happen too often, the threshold loosens; if errors are too rare, the threshold tightens. Over time this drives the empirical error rates toward their targets.  

\subsection{Theoretical Guarantees}

We now summarize the main guarantees of the online algorithm. First, the thresholds remain bounded:  

\begin{lemma}[Parameter Boundedness]
Let the scores $s(y|x) \in [0,1]$. For any $\eta > 0$, the sequences $\{a_t\}$ and $\{b_t\}$ are bounded. Specifically, for all $t > 1$:
\[
b_t \in [-\eta\varepsilon,\; 1+\eta(1-\varepsilon)], \qquad 
a_t \in [-\eta(1-\delta),\; 1+\eta\delta].
\]
\end{lemma}

With bounded parameters, the long-run error rates converge to the desired values:  

\begin{proposition}[Finite-Sample Guarantees]
Let $N_1(T) = \sum_{t=1}^T \mathbf{1}\{Y_t \in H(X_t)\}$ and $N_2(T) = \sum_{t=1}^T \mathbf{1}\{Y_t \notin H(X_t)\}$. For any $T \ge 1$:
\[
\left| \frac{1}{N_1(T)} \sum_{t=1}^T \text{err}_{\text{CH},t} - \varepsilon \right|
\le \frac{1 + \eta \max(\varepsilon, 1-\varepsilon)}{\eta N_1(T)}, \quad
\left| \frac{1}{N_2(T)} \sum_{t=1}^T \text{err}_{\text{A},t} - (1-\delta) \right|
\le \frac{1 + \eta \max(\delta, 1-\delta)}{\eta N_2(T)}.
\]
In particular, if $N_1(T), N_2(T) \to \infty$, then almost surely
\[
\lim_{T\to\infty} \frac{1}{N_1(T)} \sum_{t=1}^T \text{err}_{\text{CH},t} = \varepsilon, \qquad
\lim_{T\to\infty} \frac{1}{N_2(T)} \sum_{t=1}^T \text{err}_{\text{A},t} = 1-\delta.
\]
\end{proposition}

Together, these results say the algorithm self-adjusts: the thresholds never blow up, and over time the fraction of CH and advantage errors converges to the desired levels $(\varepsilon,\delta)$. This kind of gaurantee is typical in online conformal literature including\cite{gibbs2021adaptiveconformalinferencedistribution,angelopoulos2023conformalpidcontroltime}. This means our method remains valid even when the data stream is non-exchangeable and the human’s strategy changes with time.


\section{Human-AI Collaborative Conformalized Quantile Regression}
We now adapt conformalized quantile regression (CQR) to the human--AI collaborative framework introduced in Section~\ref{inf_sample}. 
Recall that the goal is to produce prediction sets $C(x)$ that simultaneously satisfy the counterfactual harm and complementarity constraints:
\[
\mathbb{P}\!\left(Y \notin C(X)\mid Y\in H(X)\right) \le \varepsilon,
\qquad
\mathbb{P}\!\left(Y \in C(X)\mid Y\notin H(X)\right) \ge 1-\delta .
\]

Given any quantile regression algorithm $\mathcal{A}$, we then fit four conditional quantile functions. 
Two functions $\hat{q}_{\varepsilon_{lo}}$ and $\hat{q}_{\varepsilon_{hi}}$ estimate the lower and upper quantiles that enforce the \emph{counterfactual harm} constraint when the human is correct ($Y\in H(X)$). 
Two additional functions $\hat{q}_{\delta_{lo}}$ and $\hat{q}_{\delta_{hi}}$ enforce the \emph{complementarity} constraint when the human is incorrect ($Y\notin H(X)$). 
We pass the indicator $\mathbf{1}\{Y\in H(X)\}$ as an additional input feature during training. 
Hence we use all data are used to fit all quantile regressors, avoiding class imbalance issues.

Next, we define conformity scores that quantify how far the observed label $Y_i$ lies outside the plug-in intervals implied by the quantile functions. 
For calibration point $(X_i,Y_i,H(X_i))$, the score is
\[
S_i :=
\begin{cases}
\max\!\left\{\hat{q}_{\varepsilon_{lo}}(X_i)-Y_i,\;\; Y_i - \hat{q}_{\varepsilon_{hi}}(X_i)\right\}, & Y_i \in H(X_i), \\[1ex]
\max\!\left\{\hat{q}_{\delta_{lo}}(X_i)-Y_i,\;\; Y_i - \hat{q}_{\delta_{hi}}(X_i)\right\}, & Y_i \notin H(X_i).
\end{cases}
\]
In words, if the true label lies inside the interval, the score is non-positive; if it falls outside, the score is the magnitude of the error. 

Given the calibration set $\mathcal{D}_{\text{cal}}$, we compute empirical quantiles of the conformity scores separately for the two conditions:
\[
Q^{(\varepsilon)}_{1-\varepsilon}(S,\mathcal{I}_{\text{cal}}) := (1-\varepsilon)(1+1/|\{i: Y_i \in H(X_i)\}|)\text{-th quantile of }\{S_i: Y_i\in H(X_i)\},
\]
\[
Q^{(\delta)}_{\delta}(S,\mathcal{I}_{\text{cal}}) := (\delta)(1+1/|\{i: Y_i \notin H(X_i)\}|)\text{-th quantile of }\{S_i: Y_i\notin H(X_i)\}.
\]
Finally, for a new input $X_{test}$ with human proposal $H(X_{test})$, the HA-CQR prediction set is
\[
C(X_{n+1}) =
\begin{cases}
\big[\hat{q}_{\varepsilon_{lo}}(X_{test}) - Q^{(\varepsilon)}_{1-\varepsilon},\;\;
\hat{q}_{\varepsilon_{hi}}(X_{test}) + Q^{(\varepsilon)}_{1-\varepsilon}\big], 
& \text{if } Y \in H(X_{test}), \\[1ex]
\big[\hat{q}_{\delta_{lo}}(X_{test}) - Q^{(\delta)}_{\delta},\;\;
\hat{q}_{\delta_{hi}}(X_{test}) + Q^{(\delta)}_{\delta}\big],
& \text{if } Y \notin H(X_{test}).
\end{cases}
\]

\section{Experiments}\label{exp}

\subsection{ImageNet16H - Offline - Elani's}
We begin by outlining our experimental setup. Our goal is to empirically evaluate three different components: (i) Human Alone, (ii) AI Alone, and (iii) HAI (ours). In the Human Alone case, we consider prediction sets produced directly by human experts under different strategies. (\textcolor{red}{explain how we employ these strategies without confusing the reader that we assume we dont have probabilities}) For example, under the top-k strategy, the human provides the k labels they believe most likely to be correct. Importantly, we do not observe probabilities or confidence scores from humans and only have access to the raw set of labels they provide. In the AI Alone case, we run standard conformal prediction using the AI model exclusively, without incorporating any information provided by the human expert. Finally, in the HAI case, we apply our proposed finite-sample offline algorithm. For each of the three methods, we report the \textbf{marginal coverage} achieved as well as the \textbf{average prediction set size}. For HAI, we do not directly control the marginal coverage. Instead, the configuration of $\varepsilon$ and $\delta$—which correspond to the two conditional probabilities in our formulation—governs the trade-off between the coverage achieved and the resulting set size. We present representative settings in the main text and defer additional $(\varepsilon,\delta)$ configurations to the appendix.

Our first set of experiments is conducted on the ImageNet16H dataset. This dataset contains 32,431 predictions made by 145 human participants 
on noisy variants of 1,200 natural images from the ILSVRC-2012 benchmark. 
Each image is perturbed with one of four phase noise levels 
$\omega \in \{80, 95, 110, 125\}$, which progressively increase the difficulty 
of the classification task. The label space is restricted to $L=16$ categories. 
Following prior work, we evaluate our framework using multiple pre-trained 
classifiers that have been fine-tuned for 10 epochs, including VGG19, DenseNet161, 
GoogleNet, ResNet152, and AlexNet. In the main text we present results with VGG19, 
while results for the additional architectures are deferred to the appendix. 
All reported numbers are averaged over 10 random splits of calibration and test images.

\begin{table*}[h]
\centering
\small
\begin{subtable}{0.95\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc | cccc | cc}
\toprule
\multicolumn{9}{c}{\textbf{VGG19, $\omega$ = 125}} \\
\toprule
 & \multicolumn{2}{c|}{\textbf{Human Alone}} 
 & \multicolumn{4}{c|}{\textbf{HAI (Ours)}} 
 & \multicolumn{2}{c}{\textbf{AI Alone}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9}
Strategy & Coverage & Size 
         & Coverage & Size & $\varepsilon$ & $\delta$
         & Coverage & Size \\
\midrule
Top-2 
& $0.8008 \pm 0.0090$ & $2.00 \pm 0.00$
& $\mathbf{0.9022 \pm 0.0083}$ & $\mathbf{1.49 \pm 0.04}$ & $0.05$ & $0.70$
& $0.9072 \pm 0.0138$ & $1.65 \pm 0.07$ \\
Top-1 
& $0.7245 \pm 0.0103$ & $1.00 \pm 0.00$
& $\mathbf{0.8823 \pm 0.0134}$ & $1.36 \pm 0.07$ & $0.05$ & $0.70$
& $0.8828 \pm 0.0140$ & $1.48 \pm 0.05$ \\
\bottomrule
\end{tabular}}
%\caption{VGG19, noise = 125}
\end{subtable}

\vspace{0.4em} % small gap between subtables

\begin{subtable}{0.95\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc | cccc | cc}
\toprule
\multicolumn{9}{c}{\textbf{VGG19, $\omega$ = 95}} \\
\toprule
 & \multicolumn{2}{c|}{\textbf{Human Alone}} 
 & \multicolumn{4}{c|}{\textbf{HAI (Ours)}} 
 & \multicolumn{2}{c}{\textbf{AI Alone}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9}
Strategy & Coverage & Size 
         & Coverage & Size & $\varepsilon$ & $\delta$
         & Coverage & Size \\
\midrule
% <-- plug in numbers for this noise/model combo
Top-2 
& $0.9613 \pm 0.0061$ & $2.00 \pm 0.00$
& $\mathbf{0.9825 \pm 0.0066}$ & $\mathbf{1.77 \pm 0.44}$ & $0.01$ & $0.80$
& $0.9830 \pm 0.0061$ & $2.10 \pm 0.15$ \\
\addlinespace
Top-1 
& $0.9257 \pm 0.0060$ & $1.00 \pm 0.00$
& $\mathbf{0.9763 \pm 0.0076}$ & $1.43 \pm 0.07$ & $0.01$ & $0.80$
& $0.9755 \pm 0.0053$ & $2.27 \pm 0.21$ \\
\bottomrule
\end{tabular}}
%\caption{ResNet152, noise = 95}
\end{subtable}

\caption{\textbf{Results across different AI models and noise levels.}
Each subtable reports Human Alone, HAI (Ours), and AI Alone.
Coverage and average set size are mean $\pm$ std over 10 splits.
calibration parameters $(\varepsilon,\delta)$ only applies for HAI.}
\label{tab:imagenet-main}
\end{table*}

Table \ref{tab:imagenet-main} summarizes our findings. We observe that HAI consistently improves upon the initial human sets by raising marginal coverage, even though the algorithm does not directly target coverage. Instead, coverage emerges indirectly through the choice of calibration parameters: typically, we would like  
$\varepsilon$ to be small and 
$\delta$ to be large. In many cases HAI also \textbf{achieves smaller prediction sets} than the human input or the AI baseline. For instance, when humans provide two labels (\textit{top-2}), HAI both increases coverage (e.g., from 0.80 to 0.90) and reduces the set size (from 2.0 to 1.5). To benchmark against AI alone, we evaluate conformal prediction at the same realized coverage levels as HAI. Here we find that HAI produces noticeably smaller sets—especially in lower-noise conditions
$\omega \leq 95$ where human input is more accurate—demonstrating that our method effectively leverages human knowledge.

\subsection{LLM - Differential Medical Diagnosis}
We compare for two different AI models, one that performs significantly worse than the human expert, and one that is slightly better or equal performance than the human expert. it can be seen that the stronger model is able to get smaller sets that humans and improve the coverage, whereas the weaker model inflates the set size at the cost of the coverage gain. So the stronger the AI model, the less this trade-off.


\begin{table*}[htp!]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Human Alone}} & \multicolumn{4}{c}{\textbf{HAI (Ours)}} & \multicolumn{2}{c}{\textbf{AI Alone (GPT-4o)}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-9}
\textbf{Strategy} & \textbf{Cov.} & \textbf{Size} & \textbf{Cov.} & \textbf{Size} & \boldmath$\varepsilon$ & \boldmath$\delta$ & \textbf{Cov.} & \textbf{Size} \\
\midrule
Top-1 & 0.712 & 1.000 & 0.890 & 2.557 & 0.010 & 0.650 & 0.881 & 4.578 \\
Top-1 & 0.712 & 1.000 & 0.882 & 2.508 & 0.020 & 0.650 & 0.876 & 4.404 \\
Top-1 & 0.712 & 1.000 & 0.845 & 1.766 & 0.010 & 0.500 & 0.850 & 3.692 \\
Top-1 & 0.712 & 1.000 & 0.901 & 2.840 & 0.020 & 0.700 & 0.883 & 4.639 \\
Top-1 & 0.712 & 1.000 & 0.907 & 2.904 & 0.010 & 0.700 & 0.883 & 4.639 \\
Top-1 & 0.712 & 1.000 & 0.775 & 1.134 & 0.020 & 0.200 & 0.775 & 2.490 \\
\midrule
% --- Top-2 (new rows) ---
Top-2 & 0.867 & 1.951 & 0.897 & 2.469 & 0.010 & 0.300 & 0.881 & 4.572 \\
Top-2 & 0.867 & 1.951 & 0.927 & 3.144 & 0.010 & 0.450 & 0.895 & 9.115 \\
Top-2 & 0.867 & 1.951 & 0.940 & 3.688 & 0.010 & 0.550 & 0.933 & 22.410 \\
Top-2 & 0.867 & 1.951 & 0.932 & 3.408 & 0.010 & 0.500 & 0.905 & 13.548 \\

\bottomrule
\end{tabular}
\caption{Top-5 \((\delta,\varepsilon)\) pairs maximizing coverage gain vs. Human and size gain vs. AI. AI model for the \emph{AI Alone} column is \textbf{GPT-4o}. Means shown; standard deviations not shown.}
\label{tab:gpt4o_hai_top5}
\end{table*}

\begin{table*}[htp!]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Human Alone}} & \multicolumn{4}{c}{\textbf{HAI (Ours)}} & \multicolumn{2}{c}{\textbf{AI Alone (GPT-5-mini)}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-9}
\textbf{Strategy} & \textbf{Cov.} & \textbf{Size} & \textbf{Cov.} & \textbf{Size} & \boldmath$\varepsilon$ & \boldmath$\delta$ & \textbf{Cov.} & \textbf{Size} \\
\midrule
Top-1 & 0.712 & 1.000 & 0.869 & 1.269 & 0.020 & 0.550 & 0.880 & 1.536 \\
Top-1 & 0.712 & 1.000 & 0.876 & 1.356 & 0.010 & 0.550 & 0.889 & 1.592 \\
Top-1 & 0.712 & 1.000 & 0.853 & 1.185 & 0.020 & 0.500 & 0.855 & 1.419 \\
Top-1 & 0.712 & 1.000 & 0.910 & 1.592 & 0.020 & 0.700 & 0.911 & 1.757 \\
Top-1 & 0.712 & 1.000 & 0.916 & 1.669 & 0.010 & 0.700 & 0.916 & 1.812 \\
Top-1 & 0.712 & 1.000 & 0.759 & 0.960 & 0.150 & 0.500 & 0.760 & 0.987 \\
Top-1 & 0.712 & 1.000 & 0.775 & 0.953 & 0.100 & 0.450 & 0.775 & 1.045 \\
Top-1 & 0.712 & 1.000 & 0.806 & 0.993 & 0.050 & 0.400 & 0.809 & 1.176 \\
Top-1 & 0.712 & 1.000 & 0.770 & 0.902 & 0.050 & 0.300 & 0.766 & 1.017 \\
\midrule
% --- Top-2 (replaced with new values) ---
Top-2 & 0.868 & 1.947 & 0.953 & 2.311 & 0.010 & 0.700 & 0.953 & 2.790 \\
Top-2 & 0.868 & 1.947 & 0.935 & 1.726 & 0.020 & 0.550 & 0.938 & 2.098 \\
Top-2 & 0.868 & 1.947 & 0.911 & 1.505 & 0.020 & 0.400 & 0.909 & 1.831 \\
Top-2 & 0.868 & 1.947 & 0.926 & 1.646 & 0.020 & 0.450 & 0.926 & 1.951 \\
Top-2 & 0.868 & 1.947 & 0.942 & 1.974 & 0.010 & 0.550 & 0.943 & 2.244 \\
\bottomrule
\end{tabular}
\caption{Top \((\delta,\varepsilon)\) pairs maximizing coverage gain vs.\ Human and size gain vs.\ AI for \textbf{GPT-5-mini} with \emph{Top-1, top-2} strategy. Means shown; standard deviations not shown.}
\label{tab:gpt5mini_hai_topk1_extended}
\end{table*}


\subsection{Literature Review}
\subsubsection{Conformal Prediciton}

\paragraph{Conformal prediction (CP) for uncertainty quantification.}
The notion of prediction sets traces back to classical tolerance regions \cite{lei2017distributionfreepredictiveinferenceregression, papadopoulos2002inductive}, while modern CP provides
distribution-free, finite-sample validity by constructing sets that contain the true label with a prescribed
marginal probability \cite{vovk1999machine,10.5555/1624312.1624322,vovk2005algorithmic,wilks1941determination, scheffe1945non}.
CP is now widely used in classification and regression
\cite{romano2019conformalizedquantileregression, romano2020classificationvalidadaptivecoverage},
with a large literature on improving \emph{efficiency} (shrinking set size while preserving coverage)
via adaptive scores and related refinements \cite{fisch2024calibratedselectiveclassification, Gupta_2022, kiyani2024lengthoptimizationconformalprediction,stutz2022learningoptimalconformalclassifiers,noorani2025conformalriskminimizationvariance}.

\paragraph{CP for decision making.}
Beyond coverage guarantees, recent work uses CP to \emph{shape decisions}: conformal risk control and related
formulations target risk-sensitive objectives and safety constraints, extending CP beyond pure coverage to
operational criteria \cite{angelopoulos2025conformalriskcontrol, lindemann2023safeplanningdynamicenvironments,lekeufack2024conformaldecisiontheorysafe}.
These approaches typically fix a low-dimensional action policy class and calibrate it to meet risk targets. Recently, \cite{kiyani2025decisiontheoreticfoundationsconformal} show that

\paragraph{Human--AI assisted decision making (general).}
\textcolor{blue}{learning to defer}: A complementary line of work studies when AI should abstain and defer the decision to humans,
or how to allocate instances to humans vs.\ models to exploit complementary strengths
\citep{madras2018predictresponsiblyimprovingfairness,mozannar2021consistentestimatorslearningdefer,bansal2021does}.
These methods improve team performance by routing or sharing control, often assuming access to calibrated model
confidence and focusing on \emph{who decides} on each instance.
\textcolor{blue}{How ours is different}: We do not perform routing or abstention. Instead, we take the human's initial \emph{set} as given and
ask how to algorithmically augment it with AI so the \emph{combined prediction set} is more reliable.

\paragraph{CP for human--AI decision support.}
Closer to our setting, recent work studies prediction-set based support for human experts.
\cite{detonipredsets} design prediction sets using a greedy algorithm and show that empirically it enhances human average accuracy compared to if the human had used prediction sets constructed via conformal prediction.
\cite{pmlr-v202-straitouri23a} develop an automated decision support system that, by design, does not require experts to understand when to trust the system to improve performance based on conformal prediction sets. Moreover, \cite{elanicounterfactual} analyze decision-support systems based on prediction sets through the lens of \emph{counterfactual harm}:
a system may harm a user who would have been correct unaided; they provide conditions and procedures to bound or control
such harm using conformal risk control \citep{straitouri2022counterfactual}.
However, these works are concerned with downstream accuracy of the human expert utilizing these prediction sets and do not explicitly look at collaborative uncertainty quantification where the human expert and AI model should jointly construct a prediction set. 

\paragraph{Ensemble of conformal predictors}
Another line of work considers how to combine multiple conformal predictors into a single ensemble.
\appendix
\section{Appendix}
You may include other additional sections here.
\bibliographystyle{iclr2026_conference}
\bibliography{iclr2026/iclr2026_conference}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

